OpenHealth: Open Source Platform for Wearable Health Monitoring

Movement disorders are becoming one of the leading causes of functional disability due to aging populations and extended life expectancy. Wearable health monitoring is emerging as an effective way to augment clinical care for movement disorders. However, wearable devices face a number of adaptation and technical challenges that hinder their widespread adoption. To address these challenges, we introduce OpenHealth, an open source platform for wearable health monitoring. OpenHealth aims to design a standard set of hardware/software and wearable devices that can enable autonomous collection of clinically relevant data. The OpenHealth platform includes a wearable device, standard software interfaces and reference implementations of human activity and gesture recognition applications.

==> files/opensource_requirements.tex <==
\section{Open Source Wearable Platform}
A number of wearable devices for health monitoring have been proposed in the 
last decade. Some of the recent examples include the PKG 
system\footnote{https://www.globalkineticscorporation.com.au/the-pkg-system/}
and MySignals eHealth\footnote{http://www.my-signals.com}.
 However, as noted by 
the work in~\cite{espay2016technology}, most of these devices operate in 
``competing islands of expertise'' with limited compatibility among the 
systems. 
Furthermore, most existing solutions have proprietary hardware and/or software 
that contributes to the non-compatibility among the systems. Therefore, we 
propose an open source wearable platform for health monitoring. Open source 
development 
can lead to a rapid innovation and advances, as has been shown in the machine 
learning research. To this end, an open source wearable platform has the 
following major requirements to meet the needs of patients, health 
professionals~(HP) and developers.

\subsection{Requirements for Health Monitoring}
\noindent \textbf{Modularity:} 
Most health monitoring wearable devices for movement disorders use 
accelerometer and gyroscopes to measure motion. These devices can be used to 
monitor motor symptoms in patients with movement disorders.
However, in order to monitor nonmotor symptoms, sensors such as 
sweat sensors, skin conductance sensors, blood pressure sensors are 
needed~\cite{espay2016technology}.
To fulfill these future requirements, the wearable platform needs to be modular 
in hardware and software. Hardware modularity allows for addition of new 
sensors and processing elements in the future. In order to enable modularity, 
the 
platform needs to have interfaces that allow easy addition of new modules. 
More specifically, the wearable 
platform should include hardware interfaces like SPI, which allows addition of 
new devices. Similarly, the software used in the wearable platform should be 
easily expandable to process data from new sensors and processing elements.


%For 
%example, most health monitoring wearable devices available today use 
%accelerometer and 
%gyroscopes to measure 
%motion. This can be used to monitor motor symptoms in patients with movement 
%disorders. However, in order to monitor nonmotor symptoms, sensors such as 
%sweat sensors, skin conductance sensors, blood pressure sensors are 
%needed~\cite{espay2016technology}. 
%\begin{itemize}
%	\item Expandability in hardware and software. Have interfaces that enable 
%	addition of new sensors or modules.
%	\item Similarly, software should be easily expandable to include new 
%	computing methodologies.
%\end{itemize}




\vspace{2mm}
\noindent\textbf{Scalability:}
A single device that integrates all the required sensors and processing 
elements has advantages due to its comfort, ease of use and implementation. 
This is 
because a single device can have all the sensor data and processing in a single 
location, eliminating the need to transfer large amounts of data~(local 
processing and storage requirement). However, in 
many situations a network of sensors and processing elements is better suited 
for obtaining data from different parts of the body.
% and enable additional 
%functions.
For example, to monitor both gait and heart rate of a PD patient, it is 
necessary to place sensors on the legs and hand. Therefore, the wearable 
platform should be easily scalable to include multiple devices. In order to be 
achieve the 
scalability, the platform must have synchronization between the networked 
devices and sensors. Similarly, it should support communication protocols that 
allow for efficient and low-power communication between the devices in the 
network. In addition to communication between nodes of the network, the 
wearable platform should have the ability to notify patients and HPs in case of 
an emergency. This requirement was echoed by the patients in the study 
conducted 
in~\cite{ozanne2018wearables}. In summary, the wearable platform needs to be 
easily scalable through networking, synchronization and communication protocols.
 
%\begin{itemize}
%\item One device has its advantages, however more data could enable more 
%functions
%\item Platform should be easily scalable to include more device. Create a 
%network
%\item Synchronization between devices
%\item Networking to allow efficient communication between the devices in the 
%network
%\end{itemize}
\vspace{2mm}
\noindent\textbf{Security and Privacy:}
With the rise of big data and cloud computing, increasing amount of data is 
being sent to the cloud for processing~\cite{farahani2018towards}. As a result, 
there are concerns about 
the security and privacy of the data. In the context of health monitoring, raw 
sensor data from patients is transferred to the cloud for identification of 
TOMs. The results are then communicated back to the wearable 
device. This can cause security pitfalls as the sensor data contains 
sensitive information about the patient's 
health. For instance, the patients surveyed in~\cite{ozanne2018wearables} 
expressed that data privacy and security is one of their primary concerns about 
using wearable devices for health monitoring. Therefore, the wearable platform 
should provide the highest levels of security for the data recorded from the 
users.

%\begin{itemize}
%	\item Users in previous studies expressed concerns about data security and 
%	privacy
%	\item It is critical to maintain data integrity and privacy
%\end{itemize}



\vspace{2mm}
\noindent\textbf{Local Processing and Storage:}
The open source wearable platform should include local processing and storage 
such that transfer of data to a host or the cloud is minimized. This has 
several advantages when compared to a system with no local processing. 
First, local processing and storage will allow for a faster processing of 
TOMs, as the communication latency of transferring the data to an external 
device is eliminated, leading to a better response time. Low response time is 
important for movement disorder patients such that emergencies like falls or 
seizures can be reported to care givers in real time.
Secondly, it will reduce the power consumption caused due to the transfer of a 
large amount of raw data. This will lead to significant savings, as 
communication energy is one of the major energy components in wearable
devices~\cite{asu_tech_report}. 
Finally, data security and privacy is enhanced since the 
sensor data never leaves the wearable device. 

\vspace{2mm}
\noindent\textbf{Form factor:}
Form factor is one of the most important considerations for ease of use and 
convenience of the users. The patients surveyed in~\cite{ozanne2018wearables} 
expressed the need for devices that are attractive in design and easy to wear 
under clothes. 
Furthermore, the device should be easy to wear and take off for patients with 
limited motor skills~\cite{ozanne2018wearables}.
To meet these needs, the wearable platform should be flexible 
and strive to use comfortable materials. Flexibility will allow the device to 
conform and bend according to the needs of the users. Similarly, comfortable 
materials will allow the patients to wear the device for long periods without 
feeling uncomfortable~\cite{johansson2018wearable}. In addition to 
these requirements, it is 
desirable to have properties such as water and dust resistance such that the 
device can be used in a variety of environments.
%In summary, wearable platforms 
%that are comfortable and easy to use can help in improving patience compliance 
%and adherence.  


\vspace{2mm}
\noindent\textbf{Energy efficiency and harvesting:}
One of the major considerations for health monitoring is that the 
device operate continuously with minimal interactions from the user. This is 
particularly important for movement disorders as patients with reduced motor 
skills may have difficulties in changing 
batteries~(Section~\ref{sec:barriers}). As a 
result, the wearable platform should be able to operate for long periods 
without the need to recharge the device. High capacity batteries can enable a 
longer lifetime for the device, however, they are not suitable for wearable 
applications due to their weight, size, and lack of 
comfort to users~\cite{ozanne2018wearables}. On the other hand, 
flexible batteries with comfort and form factor advantages have modest 
capacities, making them unsuitable for long term usage.
Due to these reasons, it is critical for the wearable platform to have an 
energy efficient operation.
Furthermore, the wearable platform should support energy harvesting from 
ambient sources including sunlight, body heat and body motion.
 

\vspace{2mm}
\noindent\textbf{User base and community:}
Open source wearable platforms should be supported by a community of health 
professionals, patients, hardware and software developers. These diverse 
populations need to work together to enable the widespread adoption of wearable 
health monitoring devices. This is in contrast to the current process of 
wearable device development shown in Figure~\ref{fig:health_scenario}a. In the 
current clinical 
environment, a wearable device is usually provided to patients by their HP. 
Then, the patients provide feedback to the doctors about their experience with 
the wearable device. However, there is only a loose connection between device 
manufacturers and patients who use the device. This may lead to a disconnect 
between the needs of the patients and the capabilities of the devices being 
manufactured. Therefore, all the stakeholders in the wearable health monitoring 
scenario need to work in close connection to have the maximum benefit to 
patients.

To bridge these gaps in the current wearable device development, we 
propose a development cycle shown in Figure~\ref{fig:health_scenario}b. As a 
first step in this flow, health professionals identify the 
technology-based objective measures~(TOMs) and other needs for the wearable 
platforms. 
Hardware and software developers use these objectives to design the wearable 
device. Once the hardware is available, it goes through a quality 
assessment~(QA) 
stage involving both HPs and developers. At the end of the QA stage, the device 
is provided to patients who are the end users of the device. The patients 
provide further feedback to HPs based on their real world usage of the 
device, which is incorporated in the future revisions of the wearable platform. 
This holistic approach will enable the development of wearable platforms that 
cater to the needs of both patients and health professionals.


